Transformer-Based Multi-Object Smoothing with Decoupled Data Association and Smoothing

Multi-object tracking (MOT) is the task of estimating the state trajectories of an unknown and time-varying number of objects over a certain time window. Several algorithms have been proposed to tackle the multi-object smoothing task, where object detections can be conditioned on all the measurements in the time window. However, the best-performing methods suffer from intractable computational complexity and require approximations, performing suboptimally in complex settings. Deep learning based algorithms are a possible venue for tackling this issue but have not been applied extensively in settings where accurate multi-object models are available and measurements are low-dimensional. We propose a novel DL architecture specifically tailored for this setting that decouples the data association task from the smoothing task. We compare the performance of the proposed smoother to the state-of-the-art in different tasks of varying difficulty and provide, to the best of our knowledge, the first comparison between traditional Bayesian trackers and DL trackers in the smoothing problem setting.

==> paper/conclusion.tex <==
\section{CONCLUSION}
\label{sec:conclusion}
In this study, we present what is, to the best of our knowledge, the first comprehensive comparison of the capabilities of DL-based smoothers to traditional Bayesian RFS alternatives in the model-based setting. We propose a novel, high-performing DL smoothing model, based on the transformer architecture. This model decouples the data association and smoothing subtasks, and we provide novel losses to separately supervise them. Our results show that DL models for smoothing are capable of outperforming traditional Bayesian smoothers in complicated tasks, and deteriorate in performance considerably slower than such methods as the challenge level increases.
